Oscillatory behavior in the quiet Sun observed with the New Solar Telescope

Surface photometry of the quiet Sun has achieved an angular resolution of $0".1$ with the New Solar Telescope at Big Bear Solar Observatory revealing that a disproportionate fraction of the oscillatory events appear above observed bright point-like structures. During the tracking of these structures, we noted that the more powerful oscillatory events are cospatial with them, indicating that observed flux tubes may be the source of many observed oscillatory events.

==> mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%yu-navodnik-pocetni
\def\navb{\char'134}                                      %yu-navodnik-krajnji
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} % Sasinci
\def\CJ{\' C} \def\cj{\' c} % Cicevac
\def\CH{\v C} \def\ch{\v c} % Xaxak
\def\Z{\v Z} \def\z{\v z} % Zuzemberk
\def\br{\break}


